A Gradient-Based Optimization Method Using the Koopman Operator

In this paper, we propose a novel approach to solving optimization problems by reformulating the optimization problem into a dynamical system, followed by the adaptive spectral Koopman (ASK) method. The Koopman operator, employed in our approach, approximates the evolution of an ordinary differential equation (ODE) using a finite number of eigenfunctions and eigenvalues. We begin by providing a brief overview of the Koopman operator and the ASK method. Subsequently, we adapt the ASK method for solving a general optimization problem. Moreover, we provide an error bound to aid in understanding the performance of the proposed approach, marking the initial step in a more comprehensive numerical analysis. Experimentally, we demonstrate the applicability and accuracy of our method across a diverse range of optimization problems, including min-max problems. Our approach consistently yields smaller gradient norms and higher success rates in finding critical points compared to state-of-the-art gradient-based methods. We also observe the proposed method works particularly well when the dynamical properties of the system can be effectively modeled by the system's behaviors in a neighborhood of critical points.

==> shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
% Additional Preamble
\usepackage{amsmath, amsfonts, amsopn, mathrsfs, xcolor}
\usepackage{hyperref, cleveref}
\usepackage{graphicx, epstopdf,subfigure}
\usepackage{caption, subcaption, booktabs, float, multirow}
\usepackage{algorithm, algorithmic}
\usepackage{enumerate}
\usepackage{MnSymbol}
\usepackage{lipsum}
\usepackage{bm}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Koopman Optimization}{Mengqi Hu, Bian Li, Yifei Lou, Xiu Yang}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Koopman Optimization\thanks{Submitted to the editors DATE.
\funding{
XY was supported by National Science Foundation (NSF) CAREER DMS-2143915. 
%the U.S. Department of Energy (DOE), Office of Science, Office of Advanced Scientific Computing Research (ASCR) as part of Multifaceted Mathematics for Rare, Extreme Events in Complex Energy and Environment Systems (MACSER).
BL was partially supported by (LANL LDRD).
}}}

% Authors: full names plus addresses.
\author{
Mengqi Hu\thanks{Department of Industrial and Systems Engineering, Lehigh University, Bethlehem, PA 
  (\email{meh621@lehigh.edu}, \email{bil215@lehigh.edu}, \email{xiy518@lehigh.edu})}
\and
Bian Li\footnotemark[2]
\and 
Xiu Yang\footnotemark[2]
\and 
Yifei Lou\thanks{Department of Mathematical Sciences, University of Texas at Dallas, Richardson, TX
  (\email{yifei.lou@utdallas.edu.edu})}
}

% Add user-defined concepts
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\dif}{\mathrm{d}}
\newcommand{\tensor}[1]{\mathbf{#1}}

\newcommand{\vphin}{\varphi^N}
\newcommand{\bvphin}{\bm{{\varphi}}^N}

\newcommand*{\argmax}{arg\,max}
\newcommand*{\argmin}{arg\,min}
\newcommand{\mr}{\mathbb{R}}
\newcommand{\mc}{\mathbb{C}}
\newcommand{\me}{\mathbb{E}}
\newcommand{\diag}{diag}
\newcommand{\vect}{vec}
\newcommand{\sech}{sech}

\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\vphi}{\varphi}
\newcommand{\bfx}{\bm{x}}
\newcommand{\bfy}{\bm{y}}
\newcommand{\bfpsi}{\bm{\psi}}
\newcommand{\bfc}{\bm{c}}
\newcommand{\bfPhi}{\bm{\Phi}}




\newcommand{\yl}[1]{\textcolor{green}{#1}}
\newcommand{\yx}[1]{\textcolor{yellow}{#1}}
\newcommand{\mq}[1]{\textcolor{cyan}{#1}}
 \newcommand{\h}[1]{\bm{#1}}

% \newcommand{\tensor}[1]{\mathbf{#1}}
\newcommand{\trans}{^\mathsf{T}}
% \newcommand{\dif}{\mathrm{d}}
\renewcommand{\thefootnote}{\fnsmbol{footnote}}

\newcommand{\ba}{\bm\alpha}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\bx}{\bm\xi}
\newcommand{\hc}{\hat{\bm c}} 
\newcommand{\ve}{\varepsilon}
\newcommand{\mn}{\mathbb{N}}
% \newcommand{\mr}{\mathbb{R}}
\newcommand{\tc}{\tilde{\bm c}} 
\newcommand\Def{\stackrel{\textrm{def}}{=}}

%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

